Transfer Learning for High-Precision Trajectory Tracking Through $\mathcal{L}_1$ Adaptive Feedback and Iterative Learning

Robust and adaptive control strategies are needed when robots or automated systems are introduced to unknown and dynamic environments where they are required to cope with disturbances, unmodeled dynamics, and parametric uncertainties. In this paper, we demonstrate the capabilities of a combined $\mathcal{L}_1$ adaptive control and iterative learning control (ILC) framework to achieve high-precision trajectory tracking in the presence of unknown and changing disturbances. The $\mathcal{L}_1$ adaptive controller makes the system behave close to a reference model; however, it does not guarantee that perfect trajectory tracking is achieved, while ILC improves trajectory tracking performance based on previous iterations. The combined framework in this paper uses $\mathcal{L}_1$ adaptive control as an underlying controller that achieves a robust and repeatable behavior, while the ILC acts as a high-level adaptation scheme that mainly compensates for systematic tracking errors. We illustrate that this framework enables transfer learning between dynamically different systems, where learned experience of one system can be shown to be beneficial for another different system. Experimental results with two different quadrotors show the superior performance of the combined $\mathcal{L}_1$-ILC framework compared with approaches using ILC with an underlying proportional-derivative controller or proportional-integral-derivative controller. Results highlight that our $\mathcal{L}_1$-ILC framework can achieve high-precision trajectory tracking when unknown and changing disturbances are present and can achieve transfer of learned experience between dynamically different systems. Moreover, our approach is able to achieve precise trajectory tracking in the first attempt when the initial input is generated based on the reference model of the adaptive controller.

==> images/L1_ILC_architecture_small.tex <==
% \usepackage{tikz}
% \usetikzlibrary{positioning, calc, arrows}


\tikzstyle{block} = [draw, rectangle, font=\footnotesize, minimum height=0.7cm, minimum width=1.4cm]
\tikzstyle{smallblock} = [draw, rectangle, font=\footnotesize, minimum height=0.7cm, minimum width=0.7cm]
\tikzstyle{sum} = [draw,circle, inner sep=0mm,minimum size=2mm]
\tikzstyle{connector} = [->]
\tikzstyle{line} = []
\tikzstyle{branch} = [circle,inner sep=0pt,minimum size=0.1mm,fill=black,draw=black]
\tikzstyle{guide} = []
\tikzstyle{every node}=[font=\footnotesize]
\tikzstyle{myarrows}=[line width=0.6mm,draw=gray,-triangle 45,postaction={draw, line width=1.5mm, shorten >=4mm, -}]

\begin{tikzpicture}[auto, >=stealth']
\footnotesize
\hspace{-0.1cm}
% node placement with matrix library: 5x4 array
\matrix[ampersand replacement=\&, row sep=0.25cm, column sep=0.27cm] {
  %
  \node[branch] (start) {}; \&  \node[branch] (b9) {};  \& \node[sum] (sum4) {}; \& \node[smallblock] (nonlinear) {$\begin{matrix} \text{Gain}\\ \text{K}\end{matrix}$}; \& \& \node[sum] (sum1) {}; \& \node[block] (LPF) {$\begin{matrix} \text{Low Pass}\\ \text{Filter}\end{matrix}$}; \& \node[branch] (b1) {}; \& \& \node[block, fill={rgb:black,1;white,2}] (ardrone) {System}; \& \& \node[branch] (b2) {}; \& \node[branch] (b5) {}; \& \& \node[branch] (end) {};\\

  \& \& \& \& \& \& \& \node[sum] (sum2) {}; \& \& \node[block] (refmodel) {$\begin{matrix} \text{Output} \\ \text{Predictor} \end{matrix}$}; \& \& \node [sum] (sum3) {}; \& \& \& \\
  
  \& \& \& \& \& \& \& \node[branch] (b3) {}; \&  \& \node[block] (parameters) {$\begin{matrix} \text{Adaptation} \\ \text{Law} \end{matrix}$}; \& \& \& \& \& \\
  
  \& \& \& \& \& \& \node[guide] (i1) {}; \& \& \& \& \& \& \node[branch] (b4) {}; \& \& \\%
  
  \node[branch] (b7) {}; \& \& \& \& \& \& \node[block] (learn) {$\begin{matrix} \text{Learning}\\ \text{Update}\end{matrix}$}; \& \& \& \node[block](estimation){Memory}; \& \& \& \node[branch] (b6) {}; \&  \\
};

% now link the nodes
\draw[connector] (start) -- node[pos=0.0] {$\tbf{r}_\text{2,j}$} (sum4);
\draw[connector] (sum4) -- (nonlinear);
\draw[connector] (nonlinear) -- (sum1);
\draw[connector] (sum1) -- (LPF);
\draw[line] (LPF) -- (b1);
\draw[connector] (b1) -- node[pos=0.6] {${u}(t)$} (ardrone);
\draw[line] (ardrone) -- (b2);
%\draw[connector] (ardrone) -| node[pos=0.95] {$-$}  (sum3);
\draw[connector] (b2) -- node[pos = -0.3] {$y_2(t)$} (end);
\draw[connector] (refmodel) -- (sum3);
\draw[connector] (sum3) |- node[pos = 0.38,swap] {$\widetilde{{y}}(t)$} (parameters);
\draw[connector] (sum2) -- (refmodel);
\draw[connector] (b1) -- (sum2);
%% \draw[connector] (v1) |- node {$\vec{v}_i$} (parameters);
\draw[line] (parameters) -- node[pos=0.45] {$\hat{\sigma}(t)$} (b3);
\draw[connector] (b3) -- (sum2);
\draw[connector] (b3) -| node[pos=0.95] {$-$} (sum1);
\draw[line] (b5) -- (b4);
\draw[connector] (b4) -| node[pos=0.96,swap] {$-$} (sum4);
\draw[line] (b4) -- (b6);
\draw[connector] (b6) -- (estimation);
\draw[myarrows] (estimation) -- (learn);
\draw[line, line width=1.5mm, color = gray, text=black] (learn) --node[near end] {$\tbf{r}_\text{2,j+1}$} (b7); %
\draw[line, line width=1.5mm, color = gray] (-4.24,-1.85) -- (-2,-1.85);
%\draw[myarrows] (b7) -- (start);
\draw[gray,line width=1.5mm,arrows={-Triangle[width=0.3cm]}] (b7)--(start);

% \draw[connector] (b3) -| ($(LPF.south) + (0.4cm, 0em)$);
%\draw[connector] (parameters) -| node[pos=0.96] {$-$} node [near end, swap]
                %   {$\widetilde{\vec{y}}_i$} (e1);
\draw[connector] ($(ardrone.east) - (0cm, 0.1cm)$) -| node[pos=0.96] {$-$} (sum3);
	
\draw [color=red,thick,dashed](-2.1,-2.6) rectangle (3.1,-1.3);
  \node at (-1.2,-2.45) [above=0mm, right=0mm] {\text{Iterative Learning Controller}};
    
\draw [color=blue,thick,dashed](-3.65,2.7) -- (0.6,2.7) -- (0.6,1.33) -- (3.7,1.33) -- (3.7,-1.2) -- (-3.65,-1.2) -- cycle;
  \node at (-3.6,2.5) [above=0mm, right=0mm] {\text{Extended $\lone$ Adaptive Controller}};
	
\node at (-2.4,2.1) [above=0mm, right=0mm] {$r_1(t)$};
	
\node at (2.45,1.5) [above=0mm, right=0mm] {$y_1(t)$};

%\draw[line] ($(ardrone.east) + (0cm, 0.15cm)$) -| node[near start] {$\psi$}(b6);
%\draw[connector] (b6) -| (nonlinear);

% % draw the snake lines with offset (using the calc library)
% \draw [connector] ($(i1) - (0.4cm, -1cm)$) -- node
%   {$s$} ($(LPF.south) - (0.4cm, 0em)$);

% \draw [connector, swap] ($(u1.east) + (0.1cm, -0.4cm)$) -- node
%   {$s$} ($(ardrone.west) - (0cm, 0.4cm)$);

\end{tikzpicture}

\vspace{-0.1cm}

% % \usepackage{tikz}
% % \usetikzlibrary{positioning, calc, arrows}

% \tikzstyle{block} = [draw, rectangle, font=\footnotesize, minimum height=0.7cm, minimum width=1.4cm]
% \tikzstyle{sum} = [draw,circle, inner sep=0mm,minimum size=2mm]
% \tikzstyle{connector} = [->]
% \tikzstyle{line} = []
% \tikzstyle{branch} = [circle,inner sep=0pt,minimum size=0.1mm,fill=black,draw=black]
% \tikzstyle{guide} = []
% \tikzstyle{every node}=[font=\footnotesize]

% \begin{tikzpicture}[auto, >=stealth']
% \footnotesize
% \hspace{-0.1cm}
% % node placement with matrix library: 5x4 array
% \matrix[ampersand replacement=\&, row sep=0.25cm, column sep=0.27cm] {
%   %
%   \node[branch] (start) {}; \& \& \node[sum] (sum4) {}; \& \node[block] (nonlinear) {$\begin{matrix} \text{DSL} \\ \text{Controller} \end{matrix}$}; \& \node[sum] (sum1) {}; \& \node[block] (LPF) {$\begin{matrix} \text{Low Pass}\\ \text{Filter}\end{matrix}$}; \& \node[branch] (b1) {}; \& \& \node[block] (ardrone) {AR.Drone}; \& \& \node[branch] (b2) {}; \& \node[branch] (b5) {}; \& \& \node[branch] (end) {};\\

%   \& \& \& \& \& \& \node[sum] (sum2) {}; \& \& \node[block] (refmodel) {$\begin{matrix} \text{Output} \\ \text{Predictor} \end{matrix}$}; \& \& \node [sum] (sum3) {}; \& \& \& \\
  
%   \& \& \& \& \& \& \node[branch] (b3) {}; \&  \& \node[block] (parameters) {$\begin{matrix} \text{Adaptation} \\ \text{Law} \end{matrix}$}; \& \& \& \& \& \\
  
%   \& \& \& \& \& \node[guide] (i1) {}; \& \& \& \& \& \& \node[branch] (b4) {}; \& \& \\
% };

% % now link the nodes
% \draw[connector] (start) -- node[pos=0.2] {$\tbf{x}_\text{des}$} (sum4);
% \draw[connector] (sum4) -- (nonlinear);
% \draw[connector] (nonlinear) -- (sum1);
% \draw[connector] (sum1) -- (LPF);
% \draw[line] (LPF) -- (b1);
% \draw[connector] (b1) -- node[pos=0.25] {$\tbf{u}_{\lone \text{des}}$} (ardrone);
% \draw[line] (ardrone) -- (b2);
% %\draw[connector] (ardrone) -| node[near end] {$\dot{\tbf{x}}$} node[pos=0.96] {$-$} (sum3);
% \draw[connector] (b2) -- node[near end] {$\tbf{x}$} (end);
% \draw[connector] (refmodel) -- (sum3);
% \draw[connector] (sum3) |- node[near start, swap] {$\widetilde{\tbf{y}}$} (parameters);
% \draw[connector] (sum2) -- (refmodel);
% \draw[connector] (b1) -- (sum2);
% %% \draw[connector] (v1) |- node {$\vec{v}_i$} (parameters);
% \draw[line] (parameters) -- node[pos=0.35] {$\hat{\mbs\sigma}$} (b3);
% \draw[connector] (b3) -- (sum2);
% \draw[connector] (b3) -| node[pos=0.95] {$-$} (sum1);
% \draw[line] (b5) -- (b4);
% \draw[connector] (b4) -| node[pos=0.96] {$-$} (sum4);
% % \draw[connector] (b3) -| ($(LPF.south) + (0.4cm, 0em)$);
% %\draw[connector] (parameters) -| node[pos=0.96] {$-$} node [near end, swap]
%                 %   {$\widetilde{\vec{y}}_i$} (e1);
% \draw[connector] ($(ardrone.east) - (0cm, 0.1cm)$) -| node[pos=0.96] {$-$} (sum3);
% %\draw[line] ($(ardrone.east) + (0cm, 0.15cm)$) -| node[near start] {$\psi$}(b6);
% %\draw[connector] (b6) -| (nonlinear);

% % % draw the snake lines with offset (using the calc library)
% % \draw [connector] ($(i1) - (0.4cm, -1cm)$) -- node
% %   {$s$} ($(LPF.south) - (0.4cm, 0em)$);

% % \draw [connector, swap] ($(u1.east) + (0.1cm, -0.4cm)$) -- node
% %   {$s$} ($(ardrone.west) - (0cm, 0.4cm)$);

% \end{tikzpicture}

% \vspace{-0.1cm}


==> images/L1_ILC_architecture_wide.tex <==
% \usepackage{tikz}
% \usetikzlibrary{positioning, calc, arrows}

\tikzstyle{block} = [draw, rectangle, font=\footnotesize, minimum height=1.0cm, minimum width=3.5cm]
\tikzstyle{smallblock} = [draw, rectangle, font=\footnotesize, minimum height=1.0cm, minimum width=0.7cm]
\tikzstyle{medblock} = [draw, rectangle, font=\footnotesize, minimum height=1.0cm, minimum width=2.5cm]
\tikzstyle{sum} = [draw,circle, inner sep=0mm,minimum size=3mm]
\tikzstyle{connector} = [->]
\tikzstyle{line} = []
\tikzstyle{branch} = [circle,inner sep=0pt,minimum size=0.1mm,fill=black,draw=black]
\tikzstyle{guide} = []
\tikzstyle{every node}=[font=\footnotesize]
\tikzstyle{myarrows}=[line width=0.6mm,draw=gray,-triangle 45,postaction={draw, line width=1.5mm, shorten >=4mm, -}]

\begin{tikzpicture}[auto, >=stealth']
\small
\hspace{-0.1cm}
% node placement with matrix library: 5x4 array
\matrix[ampersand replacement=\&, row sep=0.25cm, column sep=0.5cm] {
  %
  \node[branch] (start) {}; \&  \node[branch] (b9) {};  \& \node[sum] (sum4) {}; \& \node[smallblock] (nonlinear) {K Gain}; \& \& \node[sum] (sum1) {}; \& \node[medblock] (LPF) {$\begin{matrix} \text{Low Pass}\\ \text{Filter}\end{matrix}$}; \& \node[branch] (b1) {}; \& \& \node[block, fill={rgb:black,1;white,2}] (ardrone) {System}; \& \& \node[branch] (b2) {}; \& \node[branch] (b5) {}; \& \& \node[branch] (end) {};\\

  \& \& \& \& \& \& \& \node[sum] (sum2) {}; \& \& \node[block] (refmodel) {$\begin{matrix} \text{Output} \\ \text{Predictor} \end{matrix}$}; \& \& \node [sum] (sum3) {}; \& \& \& \\
  
  \& \& \& \& \& \& \& \node[branch] (b3) {}; \&  \& \node[block] (parameters) {$\begin{matrix} \text{Adaptation} \\ \text{Law} \end{matrix}$}; \& \& \& \& \& \\
  
  \& \& \& \& \& \& \node[guide] (i1) {}; \& \& \& \& \& \& \node[branch] (b4) {}; \& \& \\%
  
  \& \& \& \& \& \& \& \& \& \& \& \& \& \& \\
  
  \node[branch] (b7) {}; \& \& \& \& \& \& \node[block] (learn) {$\begin{matrix} \text{Learning}\\ \text{Update}\end{matrix}$}; \& \& \& \node[block](estimation){Memory}; \& \& \& \node[branch] (b6) {}; \&  \\
};

% now link the nodes
\draw[connector] (start) -- node[pos=0.0] {$\textbf{r}_\text{2,j}$} (sum4);
\draw[connector] (sum4) -- (nonlinear);
\draw[connector] (nonlinear) -- node[pos=0.5] {$r_1(t)$} (sum1);
\draw[connector] (sum1) -- (LPF);
\draw[line] (LPF) -- (b1);
\draw[connector] (b1) -- node[pos=0.0] {${u}(t)$} (ardrone);
\draw[line] (ardrone) -- (b2);
%\draw[connector] (ardrone) -| node[pos=0.95] {$-$}  (sum3);
\draw[connector] (b2) -- node[near end] {$y_2(t)$} (end);
\draw[connector] (refmodel) -- (sum3);
\draw[connector] (sum3) |- node[near start, swap] {$\widetilde{{y}}(t)$} (parameters);
\draw[connector] (sum2) -- (refmodel);
\draw[connector] (b1) -- (sum2);
%% \draw[connector] (v1) |- node {$\vec{v}_i$} (parameters);
\draw[line] (parameters) -- node[pos=0.35] {$\hat{\sigma}(t)$} (b3);
\draw[connector] (b3) -- (sum2);
\draw[connector] (b3) -| node[pos=0.95] {$-$} (sum1);
\draw[line] (b5) -- (b4);
\draw[connector] (b4) -| node[pos=0.96,swap] {$-$} (sum4);
\draw[line] (b4) -- (b6);
\draw[connector] (b6) -- (estimation);
\draw[myarrows] (estimation) -- (learn);
\draw[line, line width=1.5mm, color = gray, text=black] (learn) --node[near end] {$\textbf{r}_\text{2,j+1}$} (b7);
\draw[myarrows] (b7) -- (start);
%\draw[gray,line width=1.5mm,arrows={-triangle [width=0.3cm]}] (b7)--(start);

% \draw[connector] (b3) -| ($(LPF.south) + (0.4cm, 0em)$);
%\draw[connector] (parameters) -| node[pos=0.96] {$-$} node [near end, swap]
                %   {$\widetilde{\vec{y}}_i$} (e1);
\draw[connector] ($(ardrone.east) - (0cm, 0.1cm)$) -| node[near start, swap] {$y_1(t)$} node[pos=0.9, swap] {$-$} (sum3);
	
% (horizontal offset, height) rectangle (width, vertical offset)
% node at (horizontal offset, vertical offset)
\draw [color=red,thick,dashed](-3.9,-3.25) rectangle (6.4,-1.6);
  \node at (1.5,-3.7) [above=0mm, right=0mm] {\text{Iterative Learning Controller}};
    
\draw [color=blue,thick,dashed](-7.7,3.3) -- (1.4,3.3) -- (1.4,1.65) -- (7.1,1.65) -- (7.1,-1.4) -- (-7.7,-1.4) -- cycle;
  \node at (-7.4,3.6) [above=0mm, right=0mm] {\text{Extended $\mathrm{L}_1$ adaptive controller}};
	
% \node at (-2.4,2.1) [above=0mm, right=0mm] {$r_1(t)$};
	
% \node at (2.45,1.5) [above=0mm, right=0mm] {$y_1(t)$};

%\draw[line] ($(ardrone.east) + (0cm, 0.15cm)$) -| node[near start] {$\psi$}(b6);
%\draw[connector] (b6) -| (nonlinear);

% \draw [connector, swap] ($(u1.east) + (0.1cm, -0.4cm)$) -- node
%   {$s$} ($(ardrone.west) - (0cm, 0.4cm)$);

\end{tikzpicture}
\vspace{-0.9cm}
